Differentially Private Selection from Secure Distributed Computing

Given a collection of vectors $x^{(1)},\dots,x^{(n)} \in \{0,1\}^d$, the selection problem asks to report the index of an "approximately largest" entry in $x=\sum_{j=1}^n x^{(j)}$. Selection abstracts a host of problems--in machine learning it can be used for hyperparameter tuning, feature selection, or to model empirical risk minimization. We study selection under differential privacy, where a released index guarantees privacy for each vectors. Though selection can be solved with an excellent utility guarantee in the central model of differential privacy, the distributed setting lacks solutions. Specifically, strong privacy guarantees with high utility are offered in high trust settings, but not in low trust settings. For example, in the popular shuffle model of distributed differential privacy, there are strong lower bounds suggesting that the utility of the central model cannot be obtained. In this paper we design a protocol for differentially private selection in a trust setting similar to the shuffle model--with the crucial difference that our protocol tolerates corrupted servers while maintaining privacy. Our protocol uses techniques from secure multi-party computation (MPC) to implement a protocol that: (i) has utility on par with the best mechanisms in the central model, (ii) scales to large, distributed collections of high-dimensional vectors, and (iii) uses $k\geq 3$ servers that collaborate to compute the result, where the differential privacy holds assuming an honest majority. Since general-purpose MPC techniques are not sufficiently scalable, we propose a novel application of integer secret sharing, and evaluate the utility and efficiency of our protocol theoretically and empirically. Our protocol is the first to demonstrate that large-scale differentially private selection is possible in a distributed setting.

==> tex/functionality.tex <==
\subsection{Ideal Functionality}


\begin{ptbox}{$\mathcal{F}_{\text{MPC}}$}{functionality}
	\begin{description}
		\item[Private input.] Each party $i\in[n]$ has input vector $X^i\in\{0,1\}^d$. %When a party submits its input $X^i$, it is secret shared among $\numservers$ servers, each of which store $(i,X^i_j)$ for $j\in[\numservers]$. 
        The parties also agree upon a parameter $\geoparam$ for the Geometric distribution, from which noise will be sampled, as well as the divisor $\divisor$ used during truncation. It is assumed that a minority of servers $C$ of all servers $N$ are corrupt. %Also take a parameter $\truncerr$ as the possible error in the resulting truncation.
		% \item[Addition.] On inputs $X_i,X_j$, output $X_i+X_j$.
		% \item[Multiplication.] On inputs $X_i,X_j$, output $X_i\cdot X_j$.
		% \item[Comparison.] On inputs $\sum_{i\in[n]}X_i[j],\sum_{i\in[n]}X_i[k]$, output $\sum_{i\in[n]}X_i[j] > \sum_{i\in[n]}X_i[k]$.
		% \item[Approximate/Probabilistic Truncation.] Takes a parameter $\truncerr$ as the possible error in the resulting truncation. On input $X_i$ and divisor $\divisor$, output $\left\lfloor\frac{X_i}{\divisor}\right\rfloor\geq\truncate(X_i,\divisor,\truncerr)\geq\left\lfloor\frac{X_i}{\divisor}\right\rfloor-\truncerr$.
        % \item[Noise Generation.] Each server $P_j$ for $j\in[\numservers]$ generates $d$-dimensional noise $R_j$ such that each coordinate is sampled from $\text{Geo}(\geoparam)$.
		\item[Approximate/Probabilistic Argmax.] Let $(X^1,\dots,X^n)$ be the values defined by the stored values $(i,X^i)$ for $i=1,\dots,n$.
        \begin{itemize}
            \item Generate $d$-dimensional noise $|C|$ times from the negative binomial distribution with $R_j \sim \text{NB}((|N|-|C|+1)/|N|,\geoparam), j\in[|C|]$ and once for the geometric distribution with $R' \sim \text{Geo}(\geoparam)$. %where the maximal possible sum of noise values is $\maxnoise$.%Each server $P_j$ for $j\in[\numservers]$ generates $d$-dimensional noise $R_j$ such that each coordinate is sampled from $\text{Geo}(\geoparam)$.
            \item Add input values and noise as $Z=\sum_{i\in [n]}X_i+\sum_{j\in|C|}R_j + R'$, and write $Z_i$ as the $i^{th}$ entry of $Z$.
            \item For divisor $\divisor=2^\trunc$, %where $\trunc=\log(n\err-\truncerr-\maxnoise) -1$, 
            truncate entries of $Z$ with $\truncate(Z_i,\divisor,\truncerr)$, which outputs a uniform integer in range $\left[\left\lfloor\frac{Z_i}{\divisor}\right\rfloor,\left\lfloor\frac{Z_i}{\divisor}\right\rfloor-\truncerr\right]$, where $\truncerr$ depends on $\numparties$.
            \item The servers jointly compute $y^*$, where $X[y^*] = \text{max}(Z_i) \geq \text{max}(\sum_{i=1}^{n}X^i)- \err$, where $\err$ is the allowed error that depends on $|C|,\geoparam,\numparties$, and $\divisor$.
        \end{itemize}
		\item[Output.] Output the result of the evaluation $y^*$. Leak to the adversary the total number of input parties $n$, and the random noise added by corrupt parties $R_j$ for $j\in [|C|]$.	
	\end{description}
	
\end{ptbox}

\hannah{Note: with our current approach, the noise added for DP is bounded by $2^{\log(n+1)+1}$, which is very large, so alpha will also be large.}
